An Improved Analysis of Training Over-parameterized Deep Neural Networks

A recent line of research has shown that gradient-based algorithms with random initialization can converge to the global minima of the training loss for over-parameterized (i.e., sufficiently wide) deep neural networks. However, the condition on the width of the neural network to ensure the global convergence is very stringent, which is often a high-degree polynomial in the training sample size $n$ (e.g., $O(n^{24})$). In this paper, we provide an improved analysis of the global convergence of (stochastic) gradient descent for training deep neural networks, which only requires a milder over-parameterization condition than previous work in terms of the training sample size and other problem-dependent parameters. The main technical contributions of our analysis include (a) a tighter gradient lower bound that leads to a faster convergence of the algorithm, and (b) a sharper characterization of the trajectory length of the algorithm. By specializing our result to two-layer (i.e., one-hidden-layer) neural networks, it also provides a milder over-parameterization condition than the best-known result in prior work.

==> related.tex <==
\section{Related Work}
There exists a tremendous body of literature on the theory of deep learning, we are not able to conduct thorough investigation on every of them. In this section we only survey some of them which are most relevant to this paper. 

% \textbf{Representation of deep learning}
% One import topic in deep learning theory is the expressive power of deep neural network, which has been thoroughly investigated in \citet{}.

\textbf{Optimization of deep learning}
There is a vast amount of work on the optimization of deep learning. An important line of research in this topic is the landscape analysis of deep neural networks \cite{hardt2016identity,freeman2016topology,hanin2017universal,xie2017diverse,nguyen2017loss}. 

Another series of work assume that all data are generated by a ground-truth shallow network (one-hidden-layer network), or called "teacher network", and aim to establish convergence guarantees of gradient-based algorithms for recovering the ground-truth parameters \cite{tian2017analytical,brutzkus2017globally,du2017convolutional,zhong2017recovery,li2017convergence}. In particular, under the assumptions of Gaussian input and underlying teacher network, \citet{tian2017analytical} studied the convergence of gradient-based algorithms to the population loss, and pointed out there exist saddle points and local minima in population loss function. \citet{brutzkus2017sgd,du2017convolutional} further established the similar results for one-hidden-layer convolutional neural networks with ReLU activation, and proved that gradient descent is able to converge to the global minima in polynomial time when the input follows Gaussian distribution. Moreover, \citet{zhong2017recovery} further established the convergence guarantee of gradient descent for training one-hidden-layer neural network with a large class of activation functions, and showed that the training loss function enjoys local strongly convexity around the global minima. \cite{li2017convergence} considered one-hidden-layer ResNet with ReLU activation, and proved that stochastic gradient descent can converge to the global minima in two phases.


In addition to the most related work we have discussed in the introduction, there are also many efforts been made to study over-parameterized neural networks from different perspectives \cite{chizat2018note,oymak2018overparameterized,wu2019global,zhang2019training}.
\cite{oymak2018overparameterized} showed that using (stochastic) gradient descent to train a class of over-parameterized model, the iterates can be guaranteed to converge to the global minimal with a near minimal distance to the initial point.
\cite{wu2019global} studied the convergence of adaptive gradient descent for training over-parameterized one-hidden-layer ReLU network and showed that the global convergence guarantee of the proposed method does not require fine-tune learning rate. \cite{zhang2019training}
proved the global convergence rate of both gradient descent and stochastic gradient descent for training deep ResNet, and showed that the over-parameterization condition and convergence rate do not depend on the number of hidden layers.
% prove that  that given sufficiently wide neural network, both gradient descent and stochastic gradient with proper initialization can converge to the global minima of training loss function \citet{}. 


\CC{I think no need to cite generalization error papers}
\textbf{Generalization of deep learning}
We have discussed literature that reveal the dramatic power of deep neural network on the training data. Another marvelous property of deep neural network is that it can also achieve remarkable generalization performance despite its huge amount of parameters. Recently a large body of literature focused on deriving norm-based generalization error bound for deep neural networks \citep{neyshabur2015norm, bartlett2017spectrally, neyshabur2017exploring, neyshabur2017pac,  golowich2017size, neyshabur2018towards, arora2018stronger}. To name a few, \citet{bartlett2017spectrally} derived the margin-based generalization error bound based on Rademacher complexity and covering number technique. Concurrently, \citet{neyshabur2017pac} took advantage of Pac-Bayesian technique and derive a similar generalization results in terms of margin-based loss function. However, these generalization bounds was shown to be even worse than naive parameter counting \cite{arora2018convergence}. Therefore, \cite{arora2018convergence} proposed a compression framework for proving generalization bounds and showed that this can yield much tighter generalization error bound which is better than naive parameter counting.

However, these work cannot explain how the optimization algorithm affects the generalization performance of deep neural network. Therefore, this gives rise to a line of research that focuses on the algorithm-dependent generalization bound \citet{allen2018generalization,arora2019fine,cao2019generalization,yehudai2019power}. More specifically, \citet{allen2018generalization} proved that a larger shallow neural network can learn a small neural network using stochastic gradient descent up to small generalization error. \citet{arora2019fine} proved that an one-hidden-layer ReLU networks trained by gradient descent is able to learn of a broad class of smooth functions. \cite{yehudai2019power} pointed out that the optimization dynamics of training neural network behaves like learning with random features, and proved that over-parameterized one-hidden-layer ReLU networks trained by stochastic gradient descent can learn polynomials with bounded degrees and coefficients. Beyond shallow neural network, \citet{cao2019generalization} established the generalization error bound for over-parameterized deep ReLU network and proved that under certain assumptions on the data distribution, gradient descent is able to achieve arbitrary small population loss.


